Attitudes and Latent Class Choice Models using Machine learning

Latent Class Choice Models (LCCM) are extensions of discrete choice models (DCMs) that capture unobserved heterogeneity in the choice process by segmenting the population based on the assumption of preference similarities. We present a method of efficiently incorporating attitudinal indicators in the specification of LCCM, by introducing Artificial Neural Networks (ANN) to formulate latent variables constructs. This formulation overcomes structural equations in its capability of exploring the relationship between the attitudinal indicators and the decision choice, given the Machine Learning (ML) flexibility and power in capturing unobserved and complex behavioural features, such as attitudes and beliefs. All of this while still maintaining the consistency of the theoretical assumptions presented in the Generalized Random Utility model and the interpretability of the estimated parameters. We test our proposed framework for estimating a Car-Sharing (CS) service subscription choice with stated preference data from Copenhagen, Denmark. The results show that our proposed approach provides a complete and realistic segmentation, which helps design better policies.

==> sources/Limitations.tex <==
Our study also has a few limitations. Regarding our proposed model at the estimation level, the values of the latent variables change between iterations, even though the underlying structure and model probabilities are kept between runs. This is the main difference between an ML learning approach and a traditional DCM estimation, where all the parameters need to be identifiable.
On the other hand, convergence is defined empirically by setting the number of iterations due to small fluctuations in the convergence of the EM algorithm.
Also, given the small sample size, we could not divide the dataset in training, validation, and testing; therefore, the hyperparameters referring to the number of nodes and layers in the NN were not tuned according to the validation samples. %This could be solved by using a bigger dataset. 
Regarding our overall model architecture, and in order to improve the prediction performance, further work can be done, trying to apply other types of explainable AI (XAI) and other latent space representations (word embeddings) .\\
Although this work has its limitations, we are optimistic that this analysis has opened the door to future research on integrating attitudinal variables in discrete choice models through machine learning techniques. This investigation could improve the overall model fit and prediction accuracy, thanks to the representation of heterogeneity due to machine learning techniques' ability to capture complex unobserved patterns. However, we always have to bear in mind that the transparency and interpretability of new modelling frameworks are of utmost importance.
